Circuit-theoretic Joint Parameter-State Estimation -- Balancing Optimality and AC Feasibility

AC State Estimation (ACSE) is widely recognized as a practical approach for determining the grid states in steady-state conditions. It serves as a fundamental analysis to ensure grid security and is a reference for market dispatch. As grid complexity increases with rapid electrification and decarbonization, there is a growing need for more accurate knowledge of the grid operating state. However, existing ACSE algorithms have technical gaps. Critically, current ACSE algorithms are susceptible to erroneous system parameters, which are assumed to be fixed in traditional approaches. In this paper, we build a novel circuit-theoretic joint parameter-state estimation algorithm to address this limitation. The innovative algorithm builds an analogous equivalent circuit of the grid with states and certain parameters unknown. It solves a circuit-constrained optimization to estimate the most likely grid states and parameters given a set of measurements. Further, it quantifies the goodness of the estimated output by formulating tight convex envelopes around the original non-convex problem to quantify the quality of estimates. We compare the various proposed approaches on systems with up to 2869 nodes while demonstrating a tradeoff between solution optimality and model fidelity.

==> Ref.tex <==
% Generated by IEEEtran.bst, version: 1.14 (2015/08/26)
\begin{thebibliography}{10}
\providecommand{\url}[1]{#1}
\csname url@samestyle\endcsname
\providecommand{\newblock}{\relax}
\providecommand{\bibinfo}[2]{#2}
\providecommand{\BIBentrySTDinterwordspacing}{\spaceskip=0pt\relax}
\providecommand{\BIBentryALTinterwordstretchfactor}{4}
\providecommand{\BIBentryALTinterwordspacing}{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand{\BIBforeignlanguage}[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else
\language=\csname l@#1\endcsname
\fi
#2}}
\providecommand{\BIBdecl}{\relax}
\BIBdecl

\bibitem{Abur2004}
A.~Abur and A.~G. Exposito, \emph{Power system state estimation: theory and
  implementation}.\hskip 1em plus 0.5em minus 0.4em\relax CRC press, 2004.

\bibitem{Merrill1971}
H.~M. Merrill and F.~C. Schweppe, ``Bad data suppression in power system static
  state estimation,'' \emph{IEEE Transactions on Power Apparatus and Systems},
  no.~6, pp. 2718--2725, 1971.

\bibitem{Zanni2020}
L.~Zanni, A.~Dervi{\v{s}}kadi{\'c}, M.~Pignati, C.~Xu, P.~Romano, R.~Cherkaoui,
  A.~Abur, and M.~Paolone, ``Pmu-based linear state estimation of lausanne
  subtransmission network: Experimental validation,'' \emph{Electric Power
  Systems Research}, vol. 189, p. 106649, 2020.

\bibitem{Jovicic2020}
A.~Jovicic and G.~Hug, ``Linear state and parameter estimation for power
  transmission networks,'' in \emph{2020 International Conference on
  Probabilistic Methods Applied to Power Systems (PMAPS)}.\hskip 1em plus 0.5em
  minus 0.4em\relax IEEE, 2020, pp. 1--6.

\bibitem{Vanin2023}
M.~Vanin, F.~Geth, R.~D’hulst, and D.~Van~Hertem, ``Combined unbalanced
  distribution system state and line impedance matrix estimation,''
  \emph{International Journal of Electrical Power \& Energy Systems}, vol. 151,
  p. 109155, 2023.

\bibitem{Schweppe1970}
F.~C. Schweppe and J.~Wildes, ``Power system static-state estimation, part i:
  Exact model,'' \emph{IEEE Transactions on Power Apparatus and systems},
  no.~1, pp. 120--125, 1970.

\bibitem{Zhao2023}
H.~Zhao, ``A new state estimation model of utilizing pmu measurements,'' in
  \emph{2006 International Conference on Power System Technology}.\hskip 1em
  plus 0.5em minus 0.4em\relax IEEE, 2006, pp. 1--5.

\bibitem{Costa2022}
L.~F. Costa, J.~S. Giraldo, and C.~A. Castro, ``Identification and correction
  of transmission line parameter errors using scada and synchrophasor
  measurements,'' \emph{International Journal of Electrical Power \& Energy
  Systems}, vol. 135, p. 107509, 2022.

\bibitem{weng2016robust}
Y.~Weng, R.~Negi, C.~Faloutsos, and M.~D. Ili{\'c}, ``Robust data-driven state
  estimation for smart grid,'' \emph{IEEE Transactions on Smart Grid}, vol.~8,
  no.~4, pp. 1956--1967, 2016.

\bibitem{zhang2019real}
L.~Zhang, G.~Wang, and G.~B. Giannakis, ``Real-time power system state
  estimation and forecasting via deep unrolled neural networks,'' \emph{IEEE
  Transactions on Signal Processing}, vol.~67, no.~15, pp. 4069--4077, 2019.

\bibitem{sdp_acse}
Y.~Weng, Q.~Li, R.~Negi, and M.~Ilić, ``Semidefinite programming for power
  system state estimation,'' in \emph{2012 IEEE Power and Energy Society
  General Meeting}, 2012, pp. 1--8.

\bibitem{conic_acse}
Y.~Zhang, R.~Madani, and J.~Lavaei, ``Conic relaxations for power system state
  estimation with line measurements,'' \emph{IEEE Transactions on Control of
  Network Systems}, vol.~5, no.~3, pp. 1193--1205, 2017.

\bibitem{CircuitTheoretic2020}
S.~Li, A.~Pandey, S.~Kar, and L.~Pileggi, ``A circuit-theoretic approach to
  state estimation,'' in \emph{2020 IEEE PES Innovative Smart Grid Technologies
  Europe (ISGT-Europe)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2020, pp.
  1126--1130.

\bibitem{Chen2015btACOPF}
C.~Chen, A.~Atamtürk, and S.~S. Oren, ``Bound tightening for the alternating
  current optimal power flow problem,'' \emph{IEEE Transactions on Power
  Systems}, vol.~31, no.~5, pp. 3729--3736, 2016.

\bibitem{coffrin2015strengthening}
C.~Coffrin, H.~L. Hijazi, and P.~Van~Hentenryck, ``Strengthening convex
  relaxations with bound tightening for power network optimization,'' in
  \emph{International conference on principles and practice of constraint
  programming}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2015, pp.
  39--57.

\bibitem{Nagarajan2016}
H.~Nagarajan, M.~Lu, E.~Yamangil, and R.~Bent, ``Tightening mccormick
  relaxations for nonlinear programs via dynamic multivariate partitioning,''
  in \emph{Principles and Practice of Constraint Programming: 22nd
  International Conference, CP 2016, Toulouse, France, September 5-9, 2016,
  Proceedings 22}.\hskip 1em plus 0.5em minus 0.4em\relax Springer, 2016, pp.
  369--387.

\bibitem{jovicic2020enhanced}
A.~Jovicic, M.~Jereminov, L.~Pileggi, and G.~Hug, ``Enhanced modelling
  framework for equivalent circuit-based power system state estimation,''
  \emph{IEEE Transactions on Power Systems}, vol.~35, no.~5, pp. 3790--3799,
  2020.

\bibitem{Jovicic2020linear}
A.~Jovicic and G.~Hug, ``Linear state estimation and bad data detection for
  power systems with rtu and pmu measurements,'' \emph{IET Generation,
  Transmission \& Distribution}, vol.~14, no.~23, pp. 5675--5684, 2020.

\bibitem{Jovicic2019}
A.~Jovicic, M.~Jereminov, L.~Pileggi, and G.~Hug, ``A linear formulation for
  power system state estimation including rtu and pmu measurements,'' in
  \emph{2019 IEEE PES Innovative Smart Grid Technologies Europe
  (ISGT-Europe)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2019, pp. 1--5.

\bibitem{McCormick1976}
G.~P. McCormick, ``Computability of global solutions to factorable nonconvex
  programs: Part i—convex underestimating problems,'' \emph{Mathematical
  programming}, vol.~10, no.~1, pp. 147--175, 1976.

\bibitem{Javadi2021}
M.~S. Javadi, C.~S. Gouveia, L.~M. Carvalho, and R.~Silva, ``Optimal power flow
  solution for distribution networks using quadratically constrained
  programming and mccormick relaxation technique,'' in \emph{2021 IEEE
  International Conference on Environment and Electrical Engineering and 2021
  IEEE Industrial and Commercial Power Systems Europe (EEEIC/I\&CPS
  Europe)}.\hskip 1em plus 0.5em minus 0.4em\relax IEEE, 2021, pp. 1--6.

\bibitem{Bynum2018}
M.~Bynum, A.~Castillo, J.-P. Watson, and C.~D. Laird, ``Tightening mccormick
  relaxations toward global solution of the acopf problem,'' \emph{IEEE
  Transactions on Power Systems}, vol.~34, no.~1, pp. 814--817, 2018.

\bibitem{jovicic2021computationally}
A.~Jovicic, ``Computationally efficient state estimation for power systems with
  conventional and synchrophasor measurements,'' Ph.D. dissertation, ETH
  Zurich, 2021.

\end{thebibliography}

